AVATAR -- Machine Learning Pipeline Evaluation Using Surrogate Model

The evaluation of machine learning (ML) pipelines is essential during automatic ML pipeline composition and optimisation. The previous methods such as Bayesian-based and genetic-based optimisation, which are implemented in Auto-Weka, Auto-sklearn and TPOT, evaluate pipelines by executing them. Therefore, the pipeline composition and optimisation of these methods requires a tremendous amount of time that prevents them from exploring complex pipelines to find better predictive models. To further explore this research challenge, we have conducted experiments showing that many of the generated pipelines are invalid, and it is unnecessary to execute them to find out whether they are good pipelines. To address this issue, we propose a novel method to evaluate the validity of ML pipelines using a surrogate model (AVATAR). The AVATAR enables to accelerate automatic ML pipeline composition and optimisation by quickly ignoring invalid pipelines. Our experiments show that the AVATAR is more efficient in evaluating complex pipelines in comparison with the traditional evaluation approaches requiring their execution.

==> sections/old_3.motivation.tex <==

\section{Motivation}
\label{sec:mov}

To investigate the impact of invalid pipelines which are generated during the composition and optimisation, we have first conducted a series of experiments with current state-of-the-art AutoML tools.
 

\subsection{Experimental settings}

Table \ref{tab:exp_datasets} summarises characteristics of datasets used for experiments. We use these datasets because they were used in the previous studies \cite{sabu18,fekl15,olmo16}. 
The AutoML tools used for the experiments are AutoWeka4MCPS \cite{sabu18}, Auto-sklearn \cite{fekl15} and TPOT \cite{olmo16}. These tools are selected because their abilities to construct and optimise hyperparameters of complex ML pipelines have been empirically proved to be effective in a number of previous studies \cite{baal18,qume18,sabu18}. However, these previous experiments had not investigated the impact of the evaluation of invalid pipelines on the quality of the pipeline composition and optimisation yet. This is the goal of our first set of experiments.
We run the experiments on AWS EC2 $t3a.small$ virtual machines which have 2 vCPU and 2GB memory. We set the time budget to 1 hour, the memory to 1GB, and five different seed numbers for each experiment.
We independently evaluate the pipelines produced by the AutoML tools using the testing datasets and measure their predictive accuracy.




\input{tables/table_dataset_description.tex}


\subsection{Experimental results}


Figure \ref{fig:exp_accuracy_compare} compares the accuracy of the pipelines produced by AutoWeka4MCPS, TPOT and Auto-sklearn. Please refer to this supplementary document for the experimental results of TPOT and Auto-sklearn\footnote{\url{https://github.com/UTS-AAi/AVATAR/blob/master/supplementary-documents/avatar-supplementary-doc.pdf}}. We have two comments regarding these experimental results. Firstly, there are limitations of TPOT and Auto-sklearn in dealing with dirty datasets. As we can see in Figure \ref{fig:exp_accuracy_compare}, TPOT and Auto-sklearn do not produce any result for the datasets such as \textit{abalone, car} and \textit{gcredit}. The reason is that these datasets have nominal attributes and classes, and these tools can not generate pipelines that have suitable preprocessing components to deal with nominal data types. Secondly, not all of the constructed pipelines are valid. The initialisation of invalid pipelines can make the pipeline composition and optimisation methods to continue to create invalid pipelines and, in extreme cases, may not even find a valid pipeline within a time budget. 
%Thirdly, we can see that the pipeline composition and optimisation methods of AutoWeka4MCPS, TPOT and Auto-sklearn all have a degree of randomness when constructing and optimising pipelines. This randomness, as well as the generation of invalid pipelines during constructing and optimising pipelines, may lead to bad performance.
Moreover, evaluation of invalid pipelines by executing requires a large amount of time which has to be reduced.
To explore complex pipelines within a limited time budget, we propose a novel method to speed up pipeline evaluation, and thus, accelerate the pipeline composition and optimisation.
%to find better predictive models.

\begin{figure}[htb!]
\centering
\includegraphics[width=1\linewidth]{images/exp_accuracy_compare.pdf}
\caption{Comparison of the accuracy of pipelines produced by AutoWeka for MCPS, TPOT and Auto-sklearn}
\label{fig:exp_accuracy_compare}
\end{figure}


==> sections/old_4.meta_knowledge.tex <==

\section{Meta-knowledge for Constructing Machine Learning Pipelines}
\label{sec:meta_knowledge}

\subsection{Meta-features}
\label{subsec:metafeatures}

\input{tables/table_meta_features.tex}

Table \ref{tab:meta_features} describes the meta-features used for the meta-knowledge. We select these meta-features because the capabilities of a machine learning algorithm to work with a dataset depending on these meta-features of this dataset. These meta-features are extended from the capabilities of Weka algorithms. We classify these meta-features into three types as follows.

\begin{itemize}
    \item Quality: The quality type meta-features (e.g., \textit{MISSING\_VALUES}) describe quality-related characteristics of a dataset. Basically, filters can be used to improve these quality meta-features.   
    \item Attribute Transformation: The attribute transformation type meta-features (e.g., \textit{NUMERIC\_ATTRIBUTES}) describe a dataset's characteristics which can be transformed into another attribute transformation type using a filter.
    \item Class Transformation: This type of meta-feature is similar to attribute transformation. The only difference is that it is applicable for classes.
\end{itemize}








\subsection{Meta-knowledge}
\label{subsec:metaknowledge}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{images/metaknowledge_explain.pdf}
\caption{An illustration of the capabilities and the effects of a machine learning algorithm (or a pipeline's component)}
\label{fig:meta_knowledge}
\end{figure}


The purpose of the meta-knowledge is to evaluate machine learning pipelines without executing them. Therefore, a meta-knowledge of a machine learning algorithm needs to describe both this algorithm's capabilities and effects. 
Figure \ref{fig:meta_knowledge} illustrates the capabilities and effects of a machine learning algorithm. The capabilities are used to verify whether an algorithm is compatible to work with a dataset or not. For example, whether the linear regression algorithm can work with missing value and numeric attributes or not? The capabilities have a list of all meta-features described in Section \ref{subsec:metafeatures}. The value of each capability-related meta-feature is either 0 or 1.
\begin{itemize}
    \item \textit{meta-feature=0}: The algorithm can not work with the dataset which has this meta-feature.
    \item \textit{meta-feature=1}: The algorithm can work with the dataset which has this meta-feature.
\end{itemize}

Based on the capabilities, we can determine which components of a pipeline (i.e., machine learning algorithms) which are not able to work with specific meta-features of a dataset. 
On the contrary, the effects describe data transformations and data quality improvements. Similar to the capabilities, the effects have a list of all meta-features described in Section \ref{subsec:metafeatures}. Each effect-related meta-feature can have three values.

\begin{itemize}
    \item \textit{meta-feature=0}: Do not transform this meta-feature, or do not effect on this quality-related meta-feature.
    \item \textit{meta-feature=1}: Transform one or more attributes/classes to this meta-feature, or be able to improve this quality-related meta-feature.
    \item \textit{meta-feature=-1}: Disable the effect of this meta-feature on one or more attributes/classes. 
\end{itemize}

For example, \textit{EMImputation} algorithm fills in all missing values of attributes; therefore we set \textit{MISSING\_VALUES = 1} in the effects. For another example, \textit{Component Analysis} algorithm transforms nominal attributes to numeric attributes; therefore we set \textit{NUMERIC}\textit{\_ATTRIBUTES} \textit{= 1} and \textit{NOMINAL} \textit{\_ATTRIBUTES} \textit{= -1} in the effects.


%\subsection{Synthetic Datasets for Generating the Meta-knowledge}
%\label{sec:synthetic_dataset}





%Table \ref{tab:dataset} summarises characteristics of synthetic datasets which we use to generate the meta-knowledge.
%Each dataset has at least one meta-feature described in Table \ref{tab:meta_features}. 


%\input{tables/table_dataset.tex}


\subsection{Algorithm for Generating the Meta-knowledge}
\label{sec:algorithm_generating_metaknowledge}


To generate the meta-knowledge, we have to use synthetic datasets to minimise the number of active meta-features in one dataset to evaluate which and how meta-features impact on the capabilities and effects of machine learning algorithms. Real-world datasets usually have many active meta-features that make them not suitable for our purpose. We minimise the number of available meta-features in each synthetic dataset so that the meta-knowledge can be applicable in a variety of pipelines and datasets. 


\begin{itemize}
    \item Initialisation: The first stage initialises all meta-features in the capabilities and effects to 0.
    \item Execution: Run an algorithm with a synthetic dataset and get an output (i.e., an output dataset or a predictive model).
    \item Find capabilities: If the execution is successful, we set the active meta-features of the input dataset for the ones in the capabilities.
    \item Find effects: If the algorithm is a predictor/meta-predictor, we set \textit{PREDICTIVE\_MODEL} for its effects. If the algorithm is a filter and its current value is a default value, we set this effect-related meta-feature equal the difference of the values of this meta-feature of the output and input dataset. 
\end{itemize}

  

\begin{figure}[htb!]
\centering
\includegraphics[width=1\linewidth]{images/generate_metaknowledge.pdf}
\caption{Algorithm to generate the knowledge base for evaluating surrogate pipelines}
\label{fig:generate_meta_knowledge}
\end{figure}



==> sections/old_5.surrogate_validation.tex <==
\section{Surrogate Pipeline Composition and Evaluation}
\label{sec:surrogate_validation}


Because the evaluation of machine learning pipelines is expensive in certain cases (i.e., complex pipelines, high complexity pipeline's component and large datasets) in the context of AutoML, we propose AVATAR to speed up the process by evaluating their surrogate pipelines.
The main idea of AVATAR is to create a surrogate model in the form of a Petri net from its original pipeline. This surrogate pipeline keeps the structure of the pipeline, replaces the datasets in the form of data matrix (i.e., components' input/output simplified mappings) by matrices of meta-features, and the machine learning algorithms by a function to calculate the output from the input token (i.e., matrices of meta-features). Because of the simplicity of the surrogate pipeline in terms of the size of the tokens and the simplicity of the transition functions, the evaluation of this pipeline is less expensive than the original one. The implementation of AVATAR can be found here\footnote{\url{https://github.com/UTS-AAi/AVATAR}}.


\subsection{Mapping a machine learning pipeline to its surrogate model}

BPMN is the most promising method to represent an ML pipeline. The reasons are that a BPMN based ML pipeline can be executable, has a better interpretation of the pipeline in terms of control, data flows and resources for execution, as well as integrates into existing business processes as a subprocess. 
Moreover, we claim that a Petri Net is the most promising method to represent a surrogate pipeline. The reason is that it is fast to verify the validity of a Petri-net based simplified ML pipeline. Our proposed method, which generates a surrogate pipeline, has three stages, as shown in Figure \ref{fig:mapping_surrogate}.

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{images/mapping_surrogate.pdf}
\caption{Mapping a machine learning pipeline to its surrogate model}
\label{fig:mapping_surrogate}
\end{figure}

\begin{enumerate}
    \item 

   
\item Structure of the BPMN based ML pipeline is mapped to the respective structure of the Petri Net surrogate pipeline. The start and end events are mapped to the start and end places respectively. The activities are mapped to empty transitions. Empty places are put between all transitions. Finally, all flows are mapped to arcs.

\item The values of meta-features are calculated from the input dataset to form a meta-feature matrix which is the input token in the start place of the surrogate pipeline.


\item Transition functions are mapped from components. In this stage, only the corresponding algorithm information is mapped to the transition function.    
\end{enumerate}


\subsection{Evaluation of a surrogate model}

\begin{figure}[htb]
\centering
\includegraphics[width=1\linewidth]{images/fire_transition.pdf}
\caption{Algorithm for firing a transition of the surrogate model}
\label{fig:alg_transition}
\end{figure}

%\input{tables/table_component_valid_check.tex}
The evaluation of a surrogate model will execute a Petri net pipeline. This execution starts by firing each transition of the Petri net pipeline and transforming the input token.
As shown in Figure \ref{fig:alg_transition}, firing a transition consists of two tasks: (i) the evaluation of the capabilities of each component; and (ii) calculation of the output token.
The first task verifies the validity of the component using the following rules. If the value of a meta-feature stored in the input token ($m\_in\_token\_i$) is 1 and the corresponding meta-feature in the component's capabilities ($m\_cap\_i$) is 0, this component is invalid. Otherwise, this component is always valid. If a component is invalid, the surrogate pipeline is evaluated as invalid.
%For example, if the input dataset has missing values in class (i.e., MISSING\_CLASS\_VALUES=1) and the component can handle missing values in class (i.e., MISSING\_CLASS\_VALUES=1), the component is valid. 

%If the input dataset has missing values in class (i.e., MISSING\_CLASS\_VALUES=1) and the algorithm of the component cannot handle missing values in class (i.e., MISSING\_CLASS\_VALUES=0), the component is invalid. 

%If the input dataset does not have missing values in class (i.e., MISSING\_CLASS\_VALUES=0), the component is always valid.

The second task calculates each meta-feature stored in the output token (\textit{m\_out\_token\_i}) in the next place from the input token by adding the value of a meta-feature stored in the input token (\textit{m\_in\_token\_i}) and the corresponding meta-feature in the component's effects (\textit{m\_effect\_i}). 
%It is assumed that an effect-related meta-feature $X$ is MISSING\_CLASS\_VALUES. 
%For example, if the input dataset has missing values in class (i.e., $MISSING\_CLASS\_VALUES = 1$) and the component can remove/replace missing values in class (i.e., $MISSING\_CLASS\_VALUES = -1$), so that the output dataset will not have missing values in class.
%(i.e., the meta-feature of the output token is 1-1=0).

%If the input dataset has missing values in class (i.e., the meta-feature X of the input token is 1) and the algorithm of the component cannot remove/replace missing values in class (i.e., $MISSING\_CLASS\_VALUES = 0$), the output dataset still has missing values in class (i.e., the meta-feature X of the output token is 1+0=0). If the input dataset has no missing values in class (i.e., the meta-feature X of the input token is 0), the output dataset also has no missing value in class (i.e., 0-1=-1). In this case, because the values of meta-features of a dataset are either 0 or 1, the minimum value 0 is set to $MISSING\_CLASS\_VALUES$.

==> tables/table_autosklearn_experiments.tex <==

\begin{landscape}

%\begin{table*}[htb!]
\begin{table*}[htb!]

\centering


\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{}                                     & \textbf{seed=0}                                                                                                                      & \textbf{seed=1}                                                                                                                       & \textbf{seed=2}                                                                                                                       & \textbf{seed=3}                                                                                                                      & \textbf{seed=4}                                                                                                                      \\ \hline
\textbf{abalone}                  & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\textbf{amazon}                   & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\textbf{car}                      & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\multirow{3}{*}{\textbf{convex}}  & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding \\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding \\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Median\\ $\rightarrow$Feature\\ Agglomeration\\ $\rightarrow$Quantile\\ Transformer\end{tabular} \\ \cline{2-7} 
                                  & \textbf{predictor}     & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                     \\ \cline{2-7} 
                                  & \textbf{accuracy}      & 83.36                                                                                                                                & 81.84                                                                                                                                 & \textbf{83.42}                                                                                                                        & 82.73                                                                                                                                & 82.65                                                                                                                                \\ \hline
\multirow{3}{*}{\textbf{dexter}}  & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$LinearSvcPrep\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Normalize\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$LinearSvcPrep\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Normalize\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Normalize\end{tabular}                     \\ \cline{2-7} 
                                  & \textbf{predictor}     & RandomForest                                                                                                                         & SvmSvc                                                                                                                                & RandomForest                                                                                                                          & SvmSvc                                                                                                                               & SvmSvc                                                                                                                               \\ \cline{2-7} 
                                  & \textbf{accuracy}      & 93.33                                                                                                                                & \textbf{96.11}                                                                                                                        & 93.88                                                                                                                                 & 95.56                                                                                                                                & \textbf{96.11}                                                                                                                       \\ \hline
\textbf{dorothea}                 & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\textbf{gcredit}                  & -                      & -                                                                                                                                    & -                                                                                                                                     & -                                                                                                                                     & -                                                                                                                                    & -                                                                                                                                    \\ \hline
\multirow{3}{*}{\textbf{gisette}} & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean$\rightarrow$SelectRates\\ $\rightarrow$RobustScaler\end{tabular}                            & \begin{tabular}[c]{@{}l@{}}ImputationMostFrequent\\ $\rightarrow$SelectPercentile\\ $\rightarrow$Standardize\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                                               & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                                              \\ \cline{2-7} 
                                  & \textbf{predictor}     & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                      & RandomForest                                                                                                                          & RandomForest                                                                                                                         & RandomForest                                                                                                                         \\ \cline{2-7} 
                                  & \textbf{accuracy}      & \textbf{97.9}                                                                                                                        & 97.76                                                                                                                                 & 97.57                                                                                                                                 & 97.48                                                                                                                                & 97.1                                                                                                                                 \\ \hline
\multirow{3}{*}{\textbf{shuttle}} & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Standardize\end{tabular}                   & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$OneHotEncoding\\ $\rightarrow$Mean\\ $\rightarrow$Polynomial\end{tabular}                    \\ \cline{2-7} 
                                  & \textbf{predictor}     & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                      & GradientBoosting                                                                                                                     & GradientBoosting                                                                                                                     \\ \cline{2-7} 
                                  & \textbf{accuracy}      & \textbf{99.99}                                                                                                                       & 99.98                                                                                                                                 & \textbf{99.99}                                                                                                                        & \textbf{99.99}                                                                                                                       & \textbf{99.99}                                                                                                                       \\ \hline
\multirow{3}{*}{\textbf{wineqw}}  & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                 & \begin{tabular}[c]{@{}l@{}}BalancingWeighting\\ $\rightarrow$MostFreqPoly\\ $\rightarrow$RobustScaler\end{tabular}                                 \\ \cline{2-7} 
                                  & \textbf{predictor}     & Adaboost                                                                                                                             & Adaboost                                                                                                                              & Adaboost                                                                                                                              & Adaboost                                                                                                                             & Adaboost                                                                                                                             \\ \cline{2-7} 
                                  & \textbf{accuracy}      & \textbf{65.83}                                                                                                                       & \textbf{65.83}                                                                                                                        & \textbf{65.83}                                                                                                                        & \textbf{65.83}                                                                                                                       & \textbf{65.83}                                                                                                                       \\ \hline
\end{tabular}

\caption {Pipeline structure and accuracy in percentage generated by Auto-sklearn using different datasets and seed numbers}
\label{tab:autosklearn_exp}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_autoweka_experiments.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
                                   &                        & \textbf{seed=0}                                                         & \textbf{seed=1}                                                           & \textbf{seed=2}                                                                                                                    & \textbf{seed=3}                                                      & \textbf{seed=4}                                                         \\ \hline
\multirow{3}{*}{\textbf{abalone}}  & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ Ranker\end{tabular} & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular} \\ \cline{2-7} 
                                   & \textbf{predictor}     & trees.LMT                                                               & bayes.BayesNet                                                            & \begin{tabular}[c]{@{}l@{}}functions.\\ MultilayerPerceptron\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}functions.\\ SimpleLogistic\end{tabular}  & trees.LMT                                                               \\ \cline{2-7} 
                                   & \textbf{accuracy}      & 25.62                                                                   & 26.02                                                                     & \textbf{26.18}                                                                                                                     & 25.62                                                                & 25.94                                                                   \\ \hline
\multirow{3}{*}{\textbf{amazon}}   & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular} \\ \cline{2-7} 
                                   & \textbf{predictor}     & bayes.NaiveBayes                                                        & -                                                                         & rules.PART                                                                                                                         & -                                                                    & trees.J48                                                               \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{62.22}                                                          & -                                                                         & 34.67                                                                                                                              & -                                                                    & 21.78                                                                   \\ \hline
\multirow{3}{*}{\textbf{car}}      & \textbf{preprocessors} & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular} & -                                                                         & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ BestFirst\end{tabular}                                                            & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & functions.SMO                                                           & trees.J48                                                                 & functions.SMO                                                                                                                      & trees.LMT                                                            & functions.SMO                                                           \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{100.00}                                                         & 96.14                                                                     & \textbf{100.00}                                                                                                                    & 97.68                                                                & 97.68                                                                   \\ \hline
\multirow{3}{*}{\textbf{convex}}   & \textbf{preprocessors} & -                                                                       & -                                                                         & \begin{tabular}[c]{@{}l@{}}attribute.Center \rightarrow\\ attribute.PrincipalComponents\\ \rightarrow instance.PeriodicSampling\end{tabular} & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & trees.J48                                                               & -                                                                         & \begin{tabular}[c]{@{}l@{}}meta.\\ ClassificationViaRegression\end{tabular}                                                        & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{62.44}                                                          & {\ul -}                                                                   & 50.29                                                                                                                              & \textbf{-}                                                           & -                                                                       \\ \hline
\multirow{3}{*}{\textbf{dexter}}   & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & \begin{tabular}[c]{@{}l@{}}bayes.\\ NaiveBayesMultinomial\end{tabular}  & -                                                                         & -                                                                                                                                  & rules.Jrip                                                           & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{89.44}                                                          & {\ul -}                                                                   & -                                                                                                                                  & 86.67                                                                & -                                                                       \\ \hline
\multirow{3}{*}{\textbf{dorothea}} & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & rules.OneR                                                              & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{94.49}                                                          & -                                                                         & {\ul -}                                                                                                                            & -                                                                    & -                                                                       \\ \hline
\multirow{3}{*}{\textbf{gcredit}}  & \textbf{preprocessors} & -                                                                       & -                                                                         & -                                                                                                                                  & -                                                                    & \begin{tabular}[c]{@{}l@{}}attributeSelection.\\ Ranker\end{tabular}    \\ \cline{2-7} 
                                   & \textbf{predictor}     & bayes.NaiveBayes                                                        & \begin{tabular}[c]{@{}l@{}}functions.\\ MultilayerPerceptron\end{tabular} & functions.SMO                                                                                                                      & bayes.NaiveBayes                                                     & \begin{tabular}[c]{@{}l@{}}functions.\\ Logistic\end{tabular}           \\ \cline{2-7} 
                                   & \textbf{accuracy}      & 69.33                                                                   & 50.05                                                                     & 70.33                                                                                                                              & 69.33                                                                & \textbf{73.67}                                                          \\ \hline
\multirow{3}{*}{\textbf{gisette}}  & \textbf{preprocessors} & attributeSelection.Ranker                                               & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{predictor}     & trees.REPTree                                                           & -                                                                         & -                                                                                                                                  & -                                                                    & -                                                                       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{93.52}                                                          & -                                                                         & -                                                                                                                                  & -                                                                    & {\ul -}                                                                 \\ \hline
\end{tabular}


\caption {Pipeline structure and accuracy(\%) generated by AutoWeka4MCPS using different datasets and seed numbers}
\label{tab:autoweka_exp}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_capabilities.tex <==
\begin{table}[]
\begin{tabular}{l|l}
\hline
\textbf{Algorithm capability/ Dataset meta-feature} & \textbf{Description}                         \\ \hline \hline
BINARY\_ATTRIBUTES                                       & can handle binary attributes                 \\ \hline
BINARY\_CLASS                                            & can handle binary classes                    \\ \hline
DATE\_ATTRIBUTES                                         & can handle date attributes                   \\ \hline
DATE\_CLASS                                              & can handle date classes                      \\ \hline
EMPTY\_NOMINAL\_ATTRIBUTES                               & can handle empty nominal attributes          \\ \hline
EMPTY\_NOMINAL\_CLASS                                    & can handle empty nominal classes             \\ \hline
MISSING\_CLASS\_VALUES                                   & can handle missing values in class attribute \\ \hline
MISSING\_VALUES                                          & can handle missing values in attributes      \\ \hline
NOMINAL\_ATTRIBUTES                                      & can handle nominal attributes                \\ \hline
NOMINAL\_CLASS                                           & can handle nominal classes                   \\ \hline
NUMERIC\_ATTRIBUTES                                      & can handle numeric attributes                \\ \hline
NUMERIC\_CLASS                                           & can handle numeric classes                   \\ \hline
STRING\_CLASS                                            & can handle string classes                    \\ \hline
UNARY\_ATTRIBUTES                                        & can handle unary attributes                  \\ \hline
UNARY\_CLASS                                             & can handle unary classes                     \\ \hline
OUTLIER                                                  & can handle outlier                           \\ \hline
\end{tabular}

\caption {List of algorithms' capabilities or dataset meta-features}
\label{tab:capabilities}
\vspace{-0.5cm}
\end{table}

==> tables/table_component_valid_check.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Input token:\\ meta-feature X\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Algorithm\\ capability X\end{tabular}} & \textbf{Validity} \\ \hline
1                                                                              & 1                                                                         & Valid             \\ \hline
0                                                                              & 0                                                                         & Valid             \\ \hline
1                                                                              & 0                                                                         & Invalid           \\ \hline
0                                                                              & 1                                                                         & Valid             \\ \hline
\end{tabular}
\caption {Rules for checking validity of one activity/component in a pipeline}
\label{tab:component_valid}
\vspace{-0.5cm}
\end{table}

==> tables/table_dataset.tex <==
\begin{table}[htb!]
\centering



\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\#}} & \multicolumn{6}{l|}{\textbf{attributes}}                                                                  & \multicolumn{4}{l|}{\textbf{class}}                                  \\ \cline{2-11} 
                             & \textbf{n\_num} & \textbf{n\_bin} & \textbf{n\_nom} & \textbf{n\_ept} & \textbf{\%miss} & \textbf{n\_rdd} & \textbf{type} & \textbf{distinct} & \textbf{\%miss} & \textbf{distr} \\ \hline
1                            & 1               & 1               & 1               & 1               & 5\%             & 1               & nominal       & 3                 & 5\%             & 9:1            \\ \hline
2                            & 2               & 0               & 0               & 0               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
3                            & 0               & 2               & 0               & 0               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
4                            & 0               & 0               & 2               & 0               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
5                            & 1               & 0               & 0               & 1               & 0               & 0               & nominal       & 3                 & 0               & bal            \\ \hline
6                            & 2               & 0               & 0               & 0               & 5\%             & 0               & nominal       & 3                 & 0               & bal            \\ \hline
7                            & 2               & 0               & 0               & 0               & 0               & 1               & nominal       & 3                 & 0               & bal            \\ \hline
8                            & 2               & 0               & 0               & 0               & 0               & 0               & nominal       & 3                 & 5\%             & bal            \\ \hline
9                            & 2               & 0               & 0               & 0               & 0               & 0               & nominal       & 3                 & 0               & 9:1            \\ \hline
10                           & 2               & 0               & 0               & 0               & 0               & 0               & binary        & n/a               & 0               & bal            \\ \hline
11                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & n/a               & 0               & n/a            \\ \hline
12                           & 1               & 1               & 1               & 1               & 5\%             & 1               & numeric       & 3                 & 5\%             & 9:1            \\ \hline
13                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
14                           & 0               & 2               & 0               & 0               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
15                           & 0               & 0               & 2               & 0               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
16                           & 1               & 0               & 0               & 1               & 0               & 0               & numeric       & 3                 & 0               & bal            \\ \hline
17                           & 2               & 0               & 0               & 0               & 5\%             & 0               & numeric       & 3                 & 0               & bal            \\ \hline
18                           & 2               & 0               & 0               & 0               & 0               & 1               & numeric       & 3                 & 0               & bal            \\ \hline
19                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & 3                 & 5\%             & bal            \\ \hline
20                           & 2               & 0               & 0               & 0               & 0               & 0               & numeric       & 3                 & 0               & 9:1            \\ \hline
\end{tabular}



\caption {Synthetic datasets for generating meta-knowledge. Number of instances (instances), number of numeric attributes (n\_num), number of binary attributes (n\_bin), number of nominal attributes (n\_nom), number of empty attributes (n\_ept), percentage of missing values of attributes (attributes - \%miss), number of redundant attributes (n\_rdd), type of class (type), number of distinct values for nominal class (distinct), percentage of missing values of class (class - \%miss), distribution of class (distr), balance (bal), imbalanced with ratio x/y (x:y), not available (n/a).}
\label{tab:dataset}
\vspace{-0.5cm}
\end{table}

==> tables/table_exp_avatar_evaluation_time.tex <==
\begin{table}[htb!]
\caption {Comparison of the number of total evaluated, valid and invalid pipelines generated during the random search (RS), and the average evaluation time in ms of all, valid and invalid pipelines using T-method, AVATAR and AutoWeka4MCPS}
\label{tab:exp_avatar_evaluation_time}
\vspace{-0.2cm}


\resizebox{\textwidth}{!}{%
\centering

\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Total\\ evaluated\\ pipelines\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Valid\\ pipelines\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Invalid\\ pipelines\end{tabular}}} & \multicolumn{3}{l|}{\textbf{Average evaluation time (ms)}}                                                                                                                                                   \\ \cline{6-8} 
                                  &                                  &                                                                                                 &                                                                                     &                                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}All\\ pipelines\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Valid\\ pipelines\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Invalid\\ pipelines\end{tabular}} \\ \hline
\multirow{2}{*}{abalone}          & T-method                         & 72                                                                                              & 14                                                                                  & 58                                                                                    & 73,441                                                           & 176,912                                                            & 48,465                                                               \\ \cline{2-8} 
                                  & AVATAR                           & 131                                                                                             & 20                                                                                  & 111                                                                                   & 32,482                                                           & 210,908                                                            & 333                                                                  \\ \hline
\multirow{2}{*}{car}              & T-method                         & 733                                                                                             & 208                                                                                 & 525                                                                                   & 4,933                                                            & 13,362                                                             & 1,594                                                                \\ \cline{2-8} 
                                  & AVATAR                           & 891                                                                                             & 230                                                                                 & 661                                                                                   & 4,032                                                            & 14,967                                                             & 227                                                                  \\ \hline
\multirow{2}{*}{convex}           & T-method                         & 67                                                                                              & 10                                                                                  & 57                                                                                    & 53,936                                                           & 75,666                                                             & 50,124                                                               \\ \cline{2-8} 
                                  & AVATAR                           & 47                                                                                              & 9                                                                                   & 38                                                                                    & 114,791                                                          & 543,284                                                            & 13,306                                                               \\ \hline
\multirow{2}{*}{gcredit}          & T-method                         & 363                                                                                             & 102                                                                                 & 261                                                                                   & 13,451                                                           & 39,191                                                             & 3,392                                                                \\ \cline{2-8} 
                                  & AVATAR                           & 1,018                                                                                           & 244                                                                                 & 774                                                                                   & 4,663                                                            & 17,083                                                             & 748                                                                  \\ \hline
\multirow{2}{*}{wineqw}           & T-method                         & 200                                                                                             & 60                                                                                  & 140                                                                                   & 18,967                                                           & 34,988                                                             & 12,101                                                               \\ \cline{2-8} 
                                  & AVATAR                           & 549                                                                                             & 63                                                                                  & 486                                                                                   & 13,787                                                           & 101,620                                                            & 2,401                                                                \\ \hline
\end{tabular}

}


\end{table}




==> tables/table_exp_result_analyse.tex <==
\begin{table}[htb!]
\centering

\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\textbf{Configs}                                                                         & \textbf{Tools}    & \textbf{n\_best} & \textbf{n\_worst} & \textbf{n\_fail} & \textbf{min\_diff} & \textbf{max\_diff} & \textbf{avg\_diff} \\ \hline
\multirow{7}{*}{\textbf{1 hour}}                                                         & \textbf{AW}       & 2                & 0                 & 1                & \textbf{0}         & \textbf{-13.59}    & -2.63818           \\ \cline{2-8} 
                                                                                         & \textbf{AW2}      & 1                & 1                 & 1                & \textbf{0}         & -41.11             & -5.97091           \\ \cline{2-8} 
                                                                                         & \textbf{AW4MP}    & 0                & 0                 & 1                & -0.02              & -19.11             & -4.70273           \\ \cline{2-8} 
                                                                                         & \textbf{A-SKL}    & 2                & 0                 & 4                & \textbf{0}         & -39.25             & -5.675             \\ \cline{2-8} 
                                                                                         & \textbf{H2O}      & 2                & 0                 & 3                & \textbf{0}         & -41.95             & -9.32222           \\ \cline{2-8} 
                                                                                         & \textbf{TPOT}     & 1                & 0                 & 2                & \textbf{0}         & -40.38             & -6.782             \\ \cline{2-8} 
                                                                                         & \textbf{MathTC}   & 2                & 0                 & 0                & \textbf{0}         & -38.8              & -5.53083           \\ \hline
\multirow{7}{*}{\textbf{24 hours}}                                                       & \textbf{AW}       & 2                & 0                 & 0                & \textbf{0}         & -15.32             & -3.2175            \\ \cline{2-8} 
                                                                                         & \textbf{AW2}      & 1                & 0                 & 1                & \textbf{0}         & -37.33             & -6.78727           \\ \cline{2-8} 
                                                                                         & \textbf{AW4MP}    & 2                & 0                 & 0                & \textbf{0}         & -17.59             & \textbf{-2.38083}  \\ \cline{2-8} 
                                                                                         & \textbf{A-SKL}    & 2                & 0                 & 4                & \textbf{0}         & -38.58             & -5.1025            \\ \cline{2-8} 
                                                                                         & \textbf{H2O}      & 0                & 0                 & 5                & -0.15              & -44.65             & -12.38             \\ \cline{2-8} 
                                                                                         & \textbf{TPOT}     & 0                & 0                 & 2                & -0.21              & -38.13             & -6.685             \\ \cline{2-8} 
                                                                                         & \textbf{MathTC}   & 1                & 0                 & 0                & \textbf{0}         & -38.58             & -6.176             \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}No\\ time\\ constraint\end{tabular}}} & \textbf{MLBox}    & 1                & 0                 & 2                & \textbf{0}         & -40.38             & -7.377             \\ \cline{2-8} 
                                                                                         & \textbf{AutoML}   & 1                & 0                 & 0                & \textbf{0}         & -31.16             & -6.88083           \\ \cline{2-8} 
                                                                                         & \textbf{RM}       & 0                & 1                 & 0                & -0.07              & -32                & -7.24              \\ \cline{2-8} 
                                                                                         & \textbf{ATM}      & 1                & 1                 & 1                & \textbf{0}         & -41.05             & -11.0309           \\ \cline{2-8} 
                                                                                         & \textbf{AWS ML}   & 1                & 1                 & 2                & \textbf{0}         & -38.13             & -12.598            \\ \hline
\multirow{4}{*}{\textbf{Baselines}}                                                      & \textbf{NBayes}   & 0                & 5                 & 0                & -7                 & {\underline{-59.7}}        & {\underline{-25.56}}       \\ \cline{2-8} 
                                                                                         & \textbf{LogReg}   & 0                & 3                 & 0                & {\underline{-0.43}}        & -40.15             & -15.3942           \\ \cline{2-8} 
                                                                                         & \textbf{RdForest} & 1                & 0                 & 0                & \textbf{0}         & -39.7              & -7.74833           \\ \cline{2-8} 
                                                                                         & \textbf{XGBoost}  & 1                & 0                 & 0                & \textbf{0}         & -39.03             & -8.34833           \\ \hline
\end{tabular}



\caption {Experimental results of the AutoML tools: number of the best predictive models (n\_best), number of the worst predictive models (n\_worst), number of failed cases (n\_fail), minimum difference from the best predictive model (min\_diff), maximum difference from the best predictive model (max\_diff), and average difference from the best predictive model (avg\_diff)  }



\label{tab:exp_results_analyse}
\vspace{-0.5cm}
\end{table}

==> tables/table_generate_pipeline_method_compare.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering





\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Method}}                                 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Pipeline\\ structure\end{tabular}}} & \multicolumn{3}{l|}{\textbf{Max components by type}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Max\\ length\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Knowledge for\\ construction\end{tabular}}} & \multicolumn{3}{l|}{\textbf{Libraries/algorithms}}       & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Hyperparameter\\ Optimization\end{tabular}}}     \\ \cline{3-5} \cline{8-10}
                                                                 &                                                                                        & \textbf{Prep}    & \textbf{Pred}   & \textbf{Ense}   &                                                                                &                                                                                                & \textbf{Prep}            & \textbf{Pred} & \textbf{ense} &                                                                                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}Auto-weka \\ v0.5/v2.0\end{tabular}   & SW                                                                                     & 1                & 1               & 1               & 3                                                                              & fixed                                                                                          & 3                        & 36            & 0             & SMAC                                                                                                \\ \hline
\begin{tabular}[c]{@{}l@{}}Auto-weka\\ for MCPS\end{tabular}     & SW                                                                                     & 5                & 1               & 1               & 7                                                                              & fixed                                                                                          & 17                       & 34            & 0             & SMAC                                                                                                \\ \hline
Auto-sklearn                                                     & SW                                                                                     & 4                & 1               & 0               & 5                                                                              & fixed                                                                                          & 18                       & 15            & 1             & SMAC                                                                                                \\ \hline
Bolme et al.                                                     & SW                                                                                     & 1                & 1               & 0               & 2                                                                              & fixed                                                                                          & 1                        & 1             & NA            & GP                                                                                                  \\ \hline
RECIPE                                                           & \begin{tabular}[c]{@{}l@{}}derivation\\ tree\end{tabular}                              & ul               & ul              & 1               & ul                                                                             & CFG                                                                                            & 33                       & 23            & 4             & Random search                                                                                       \\ \hline
GRADIENT                                                         & tree                                                                                   & 0                & ul              & ul              & ul                                                                             & CFG                                                                                            & NA                       & NA            & NA            & GP                                                                                                  \\ \hline
TPOT                                                             & tree                                                                                   & ul               & 1               & 1               & ul                                                                             & NA                                                                                             & 19                       & 11            & 0             & \begin{tabular}[c]{@{}l@{}}Pareto\\ optimization\end{tabular}                                       \\ \hline
Layered-TPOT                                                     & tree                                                                                   & ul               & 1               & 1               & ul                                                                             & NA                                                                                             & NA                       & NA            & NA            & \begin{tabular}[c]{@{}l@{}}Pareto\\ optimization\end{tabular}                                       \\ \hline
Kordik et al.                                                    & tree                                                                                   & 0                & ul              & ul              & ul                                                                             & CFG                                                                                            & 0                        & 5             & 7             & GP                                                                                                  \\ \hline
ML-Plan                                                          & SW                                                                                     & ul               & 1               & 1               & ul                                                                             & HTN search space                                                                               & 25                       & 42            & 0             & Random search                                                                                       \\ \hline
ML-Plan-UL                                                       & SW                                                                                     & ul               & ul              & 1               & ul                                                                             & HTN search space                                                                               & 25                       & 42            & 3             & Random search                                                                                       \\ \hline
MLS-Plan                                                         & SW                                                                                     & ul               & 1               & 1               & ul                                                                             & HTN search space                                                                               & \multicolumn{3}{l|}{NA}                                  & Random search                                                                                       \\ \hline
P4ML                                                             & SW                                                                                     & yes              & yes             & yes             & NA                                                                             & \begin{tabular}[c]{@{}l@{}}A catalog \\ of primitives\end{tabular}                             & \multicolumn{1}{c|}{127} &               &               & NA                                                                                                  \\ \hline
AutoComplete                                                     & tree                                                                                   & NA               & ul              & 1               & ul                                                                             & fixed                                                                                          & NA                       & 14            & 1             & \begin{tabular}[c]{@{}l@{}}Random search \\ or grid search\end{tabular}                             \\ \hline
\begin{tabular}[c]{@{}l@{}}Automatic\\ Frankenstein\end{tabular} & tree                                                                                   & 0                & ul              & 1               & ul                                                                             & \begin{tabular}[c]{@{}l@{}}Meta-learning from \\ historical runs\end{tabular}                  & NA                       & NA            & NA            & \begin{tabular}[c]{@{}l@{}}Meta-learning\\ + model selection \\ + weighted \\ ensemble\end{tabular} \\ \hline
AutoBagging                                                      & tree                                                                                   & 0                & NA              & NA              & NA                                                                             & fixed                                                                                          & NA                       & NA            & NA            & \begin{tabular}[c]{@{}l@{}}Meta-learning \\ + average rank \\ of models\end{tabular}                \\ \hline
\end{tabular}





\caption {Comparison of the pipeline composition and optimisation methods in term of pipeline structure, max number of components by type in a pipeline (preprocessor, predictor, and ensemble), max length of a pipeline, knowledge for pipeline construction, libraries/algorithms used for implementation (preprosessor, predictor, and ensemble), hyperparameter optimisation method. SW: sequential workflow, ul: unlimited length, HTN: hierarchical task network, CFG: context free grammars, NA: not available, GP: genetic programming, fixed: fixed template.}
\label{tab:method_compare}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_io_convert.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|}
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Input token: \\ meta-feature X\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Algorithm\\ capability X\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Output token:\\ meta-feature X\end{tabular}} \\ \hline
1                                                                               & 1                                                                         & 0                                                                               \\ \hline
0                                                                               & 0                                                                         & 0                                                                               \\ \hline
1                                                                               & 0                                                                         & 1                                                                               \\ \hline
0                                                                               & 1                                                                         & 0                                                                               \\ \hline
\end{tabular}
\caption {Rules to calculate output token from input token and algorithm capabilities}
\label{tab:io_convert}
\vspace{-0.5cm}
\end{table}

==> tables/table_methods_compare.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering
%\small


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{\#}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{l|}{\textbf{Predict model}} & \multicolumn{4}{l|}{\textbf{Search space's characteristics}}         & \multicolumn{3}{l|}{\textbf{Search space tructure}} & \multicolumn{4}{l|}{\textbf{Approach to find best model}}             \\ \cline{3-15} 
                             &                                  & \textbf{Cls}          & \textbf{Regrs}         & \textbf{Prep} & \textbf{Clsfier} & \textbf{M-clsfier} & \textbf{Hyp} & \textbf{Func}   & \textbf{Tree}   & \textbf{Graph}  & \textbf{BayesOpt} & \textbf{HPlan} & \textbf{Rand} & \textbf{M-learn} \\ \hline
1                            & ROAR                             & -                     & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & -               & -               & -                 & -              & $\checkmark$  & -                \\ \hline
2                            & SMAC                             & $\checkmark$          & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
3                            & TPE                              & -                     & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
4                            & CASH                             & $\checkmark$          & $\checkmark$           & -             & $\checkmark$     & -                  & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
5                            & MCPS                             & $\checkmark$          & $\checkmark$           & $\checkmark$  & $\checkmark$     & $\checkmark$       & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & -                \\ \hline
6                            & Spearmint                        & -                     & $\checkmark$           & -             & -                & -                  & $\checkmark$ & $\checkmark$    & -               & -               & $\checkmark$      & -              & -             & -                \\ \hline
7                            & HyperBand                        & $\checkmark$          & $\checkmark$           & -             & -                & -                  & $\checkmark$ & -               & -               & -               & -                 & -              & $\checkmark$  & -                \\ \hline
8                            & ML-Plan                          & $\checkmark$          & $\checkmark$           & $\checkmark$  & $\checkmark$     & $\checkmark$       & $\checkmark$ & -               & -               & $\checkmark$    & -                 & $\checkmark$   & -             & -                \\ \hline
9                            & AR*                              & $\checkmark$          & $\checkmark$           & -             & $\checkmark$     & -                  & $\checkmark$ & -               & -               & -               & -                 & -              & -             & $\checkmark$     \\ \hline
10                           & Auto-sklearn                     & $\checkmark$          & $\checkmark$           & $\checkmark$  & $\checkmark$     & $\checkmark$       & $\checkmark$ & -               & $\checkmark$    & -               & $\checkmark$      & -              & -             & $\checkmark$     \\ \hline
\end{tabular}


\caption {Compare composition and optimisation methods for machine learning pipelines in term of predictive model type (classification or regression), characteristics of search space (preprocessing, classifier, meta-classifier and hyper-parameters), structure of search space (based on function, tree, and graph) and approaches to find best predictive models (based on Bayesian optimisation, hierarchical planning, random and meta-learning) }
\label{tab:method_compare}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_performance.tex <==
\begin{landscape}
\begin{table*}[htb!]
\centering

\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{dataset}}                                                                 & \textbf{abalone} & \textbf{amazon} & \textbf{car}    & \textbf{\begin{tabular}[c]{@{}l@{}}german\\ credit\end{tabular}} & \textbf{gisette} & \textbf{krvskp} & \textbf{madelon} & \textbf{semeion} & \textbf{shuttle} & \textbf{\begin{tabular}[c]{@{}l@{}}wave\\ form\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}wine\\ qw\end{tabular}} & \textbf{yeast} \\ \hline
\multirow{7}{*}{\textbf{1h}}                                                        & \textbf{AW}      & 22.91            & -               & 99.81           & 72.33                                                            & 97.33            & 99.48           & 73.72            & 93.50            & \textbf{99.99}   & 85.60                                                        & \textbf{67.19}                                             & 62.02          \\ \cline{2-14} 
                                                                                    & \textbf{AW2}     & 25.94            & \underline{40.22}     & \textbf{100.00} & 71.00                                                            & 95.29            & 99.58           & -                & 90.36            & 99.86            & 85.93                                                        & 63.51                                                      & 59.55          \\ \cline{2-14} 
                                                                                    & \textbf{AW4MP}    & 22.83            & 62.22           & 98.46           & 72.33                                                            & -                & 99.37           & 79.10            & 91.82            & 99.97            & 85.80                                                        & 65.21                                                      & 57.53          \\ \cline{2-14} 
                                                                                    & \textbf{A-SKL}   & -                & -               & 99.03           & \textbf{75.00}                                                   & 97.38            & 99.48           & 83.08            & 94.76            & -                & \textbf{86.33}                                               & -                                                          & 23.15          \\ \cline{2-14} 
                                                                                    & \textbf{H20}     & -                & 48.00           & 98.65           & 71.67                                                            & 97.71            & \textbf{99.79}  & -                & -                & \textbf{99.99}   & 85.33                                                        & 64.40                                                      & 20.45          \\ \cline{2-14} 
                                                                                    & \textbf{TPOT}    & 25.94            & -               & 98.65           & 73.00                                                            & -                & 99.37           & 83.97            & 92.66            & \textbf{99.99}   & 85.53                                                        & 56.09                                                      & 22.02          \\ \cline{2-14} 
                                                                                    & \textbf{MathTC}  & 25.38            & \textbf{81.33}  & 98.46           & 72.00                                                            & 97.67            & 99.16           & 82.95            & 89.52            & \textbf{99.99}   & 83.27                                                        & 64.53                                                      & 23.60          \\ \hline
\multirow{7}{*}{\textbf{24h}}                                                       & \textbf{AW}      & 26.49            & 66.01           & 99.60           & 71.76                                                            & 97.76            & 99.69           & 78.44            & \textbf{94.92}   & \textbf{99.99}   & 85.58                                                        & 66.05                                                      & 59.33          \\ \cline{2-14} 
                                                                                    & \textbf{AW2}     & 25.14            & 44.00           & \textbf{100.00}    & 70.67                                                            &                  & 99.48           & 79.23            & 87.42            & 99.86            & 86.13                                                        & 63.38                                                      & 56.4           \\ \cline{2-14} 
                                                                                    & \textbf{AW4MP}    & 26.59            & 63.74           & 99.9            & 74.58                                                            & 97.66            & 99.77           & 83.20            & 94.90            & \textbf{99.99}   & 85.83                                                        & 67.10                                                      & \textbf{62.40} \\ \cline{2-14} 
                                                                                    & \textbf{A-SKL}   & -                & -               & 99.61           & 74.67                                                            & \textbf{97.86}   & 99.58           & \textbf{87.31}   & 94.34            & -                & 85.60                                                        & -                                                          & 23.82          \\ \cline{2-14} 
                                                                                    & \textbf{H20}     & -                & 62.67           & -               & 72.67                                                            & 97.71            & -               & -                & 93.50            & -                & 85.33                                                        & 48.74                                                      & 17.75          \\ \cline{2-14} 
                                                                                    & \textbf{TPOT}    & 25.94            & -               & 97.88           & 73.00                                                            & 97.14            & 99.58           & 83.97            & 92.66            & -                & 85.53                                                        & 56.09                                                      & 24.27          \\ \cline{2-14} 
                                                                                    & \textbf{MathTC}  & 25.06            & -               & 99.42           & 71.67                                                            & -                & 99.58           & 82.95            & 90.99            & \textbf{99.99}   & 85.27                                                        & 64.53                                                      & 23.82          \\ \hline
\multirow{5}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}no\\ time\\ limit\end{tabular}}} & \textbf{MLBox}   & 24.50            & -               & 94.40           & 73.33                                                            & -                & 99.06           & 82.82            & 90.57            & \textbf{99.99}   & 83.93                                                        & 60.65                                                      & 22.02          \\ \cline{2-14} 
                                                                                    & \textbf{AutoML}  & 25.78            & 63.56           & 95.75           & 74.67                                                            & 97.33            & 99.06           & 71.67            & 91.19            & \textbf{99.99}   & 85.73                                                        & 65.69                                                      & 31.24          \\ \cline{2-14} 
                                                                                    & \textbf{RapidM}  & -                & 49.33           & 98.84           & \underline{66.33}                                                      & 96.95            & 97.39           & 81.15            & 89.10            & 99.92            & 85.40                                                        & 62.90                                                      & 45.17          \\ \cline{2-14} 
                                                                                    & \textbf{ATM}     & -                & 56.89           & 97.88           & 72.67                                                            & 96.52            & 97.29           & 67.56            & 83.23            & \textbf{99.99}   & \underline{76.20}                                                  & 61.20                                                      & 21.35          \\ \cline{2-14} 
                                                                                    & \textbf{AWS ML}  & \textbf{32.11}   & -               & 86.87           & 70.00                                                            & -                & 90.29           & \underline{52.31}      & 90.36            & 99.91            & 82.77                                                        & 50.17                                                      & 24.27          \\ \hline
\multirow{4}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}base\\ line\end{tabular}}}       & \textbf{NBayes}      & 11.33            & 48.22           & 66.02           & 68.00                                                            & \underline{74.10}      & \underline{59.81}     & 63.59            & \underline{77.15}      & \underline{82.66}      & 78.80                                                        & 45.13                                                      & \underline{2.70}     \\ \cline{2-14} 
                                                                                    & \textbf{LogReg}      & \underline{10.00}      & 74.22           & \underline{63.90}     & 67.00                                                            & 97.43            & 96.66           & 55.38            & 89.73            & 95.19            & 85.53                                                        & \underline{42.21}                                                & 22.25          \\ \cline{2-14} 
                                                                                    & \textbf{RdForest}      & 23.46            & 64.89           & 98.84           & 70.33                                                            & 97.10            & 98.85           & 72.82            & 92.03            & \textbf{99.99}   & 83.73                                                        & 66.51                                                      & 22.70          \\ \cline{2-14} 
                                                                                    & \textbf{XGBoost} & 25.86            & 70.67           & 94.21           & 70.67                                                            & 97.24            & 97.39           & 73.72            & 90.36            & \textbf{99.99}   & 83.80                                                        & 56.77                                                      & 23.37          \\ \hline
\end{tabular}


\caption {Experimental results of AutoML tools: AutoWeka v0.5 - SMAC (AW), AutoWeka v2.6.1 - SMAC (AW2), AutoWeka for MCPS - SMAC (AW4MP), Auto-sklearn (A-SKL), H20, TPOT, Mathematica (MathTC), MLBox, AutoML, RapidMiner (RapidM), ATM, AWS Machine Learning (AWS ML), Naive Bayes (NBayes), Logistic Regression (LogReg), Random Forest (RdForest) and XGBoost}
\label{tab:exp_results}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_pipeline_modeling.tex <==
\begin{table}[htb!]





\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{Method}                                                                       & \textbf{\begin{tabular}[c]{@{}l@{}}Function\\ composition\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Directed\\ acyclic\\ graphs\end{tabular}} & \textbf{Petri nets} & \textbf{OWL-S} & \textbf{BPMN} & \textbf{BPEL} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Easily\\ understandable\\ by human\end{tabular}}   & no                                                                      & yes                                                                          & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Easily\\ understandable\\ by machine\end{tabular}} & yes                                                                     & no                                                                           & no                  & no             & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Support different\\ component types\end{tabular}}  & abstract                                                                & abstract                                                                     & abstract            & no             & yes           & no            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Modeling \\ data flow\end{tabular}}                & yes                                                                     & no                                                                           & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Modeling \\ control flow\end{tabular}}             & yes                                                                     & yes                                                                          & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Modeling \\ meta-features flow\end{tabular}}       & no                                                                      & no                                                                           & no                  & yes            & no            & no            \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Validation\\ data flow\end{tabular}}               & yes                                                                     & no                                                                           & no                & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Validation\\ control flow\end{tabular}}            & yes                                                                     & yes                                                                          & yes                 & yes            & yes           & yes           \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Validating\\ meta-features flow\end{tabular}}      & no                                                                      & no                                                                           & no                  & no             & no            & no            \\ \hline
\end{tabular}





\caption {Comparison of the pipeline modelling methods using the nine selected criteria. It is possible for function composition, directed acyclic graphs and Petri nets to generate pipelines consisting of different component types, however, the execution of these component types is not supported by libraries by default. Therefore, the criterion of the three approaches is abstract.}
\label{tab:modeling_compare}
\vspace{-0.5cm}
\end{table}

==> tables/table_tools_features.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering


\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Tool}}                                 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Pipeline composition\\ or algorithm selection\end{tabular}}} & \multicolumn{5}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Hyperparameter\\ optimisation\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Programming\\ language\end{tabular}}} & \multirow{2}{*}{\textbf{Libraries}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Distributed\\ processing\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Auto\\ deployment\end{tabular}}} \\ \cline{3-7}
                                                               &                                                                                                                 & \textbf{a}         & \textbf{b}         & \textbf{c}        & \textbf{d}        & \textbf{e}        &                                                                                          &                                     &                                                                                            &                                                                                     \\ \hline
Auto-Weka 0.5                                                  & algorithm selection                                                                                             & yes                & -                  & -                 & yes               & -                 & Java, Python                                                                             & Weka                                & no                                                                                         & no                                                                                  \\ \hline
Auto-Weka 2.0                                                  & algorithm selection                                                                                             & yes                & -                  & -                 & -                 & -                 & Java, Python                                                                             & Weka                                & no                                                                                         & no                                                                                  \\ \hline
\begin{tabular}[c]{@{}l@{}}Auto-Weka \\ for MCPS\end{tabular}  & pipeline composition                                                                                            & yes                & -                  & -                 & yes               & -                 & Java, Python                                                                             & Weka                                & no                                                                                         & no                                                                                  \\ \hline
Auto-sklearn                                                   & pipeline composition                                                                                            & yes                & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
H20                                                            & algorithm selection                                                                                             & -                  & yes                & -                 & -                 & -                 & Java, Python                                                                             & -                                   & yes                                                                                        & no                                                                                  \\ \hline
TPOT                                                           & pipeline composition                                                                                            & -                  & -                  & yes               & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
Mathematica                                                    & algorithm selection                                                                                             & yes                & -                  & -                 & -                 & -                 & -                                                                                        & -                                   & no                                                                                         & no                                                                                  \\ \hline
MLBox                                                          & pipeline composition                                                                                            & yes                & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
Auto\_ml                                                       & pipeline composition                                                                                            & -                  & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & no                                                                                         & no                                                                                  \\ \hline
RapidMiner                                                     & pipeline composition                                                                                            & -                  & yes                & yes               & -                 & -                 & -                                                                                        & -                                   & yes                                                                                        & yes                                                                                 \\ \hline
ATM                                                            & pipeline composition                                                                                            & yes                & -                  & -                 & -                 & -                 & Python                                                                                   & Scikit-learn                        & yes                                                                                        & no                                                                                  \\ \hline
\begin{tabular}[c]{@{}l@{}}AWS Machine\\ Learning\end{tabular} & algorithm selection                                                                                             & -                  & -                  & -                 & -                 & yes               & -                                                                                        & -                                   & yes                                                                                        & yes                                                                                 \\ \hline
\end{tabular}


\caption {Compare AutoML tools in term of (1) Ability to automatically construct pipelines or select algorithm, (2) Hyperparameter optimisation method (a. Bayesian optimisation, b. Grid search, c. Genetic algorithm, d. Random search, e. Others), (3) Programming language, (4) Libraries used for preprocessing, classification, regression and ensemble algorithms, (5) Ability to run on distributed environment, (6) Auto deploy predictive model/pipeline and generate APIs for end users. An AutoML tool can automatically construct and optimise a pipeline including at least two components is marked as \textit{pipeline composition}, and only automatically select an algorithm and optimise its hyperparameters is marked as \textit{algorithm selection}. Symbol '-' represents for not available information.   }
\label{tab:tool_compare}
\vspace{-0.5cm}
\end{table*}


\end{landscape}

==> tables/table_tpot_experiments.tex <==
\begin{landscape}

\begin{table*}[htb!]
\centering


\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
                                   &                        & \textbf{seed=0}    & \textbf{seed=1}                                                                      & \textbf{seed=2}   & \textbf{seed=3}   & \textbf{seed=4}    \\ \hline
\multirow{3}{*}{\textbf{abalone}}  & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{amazon}}   & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{car}}      & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{convex}}   & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & RandomForest       & RandomForest                                                                         & RandomForest      & XGBoost           & GradientBoosting   \\ \cline{2-7} 
                                   & \textbf{accuracy}      & 74.14              & {\ul 73.78}                                                                          & 74.97             & \textbf{78.89}    & 78.23              \\ \hline
\multirow{3}{*}{\textbf{dexter}}   & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & MultinomialNB                                                                        & MultinomialNB     & MultinomialNB     & MultinomialNB      \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & {\ul 92.78}                                                                          & \textbf{93.33}    & \textbf{93.33}    & \textbf{93.33}     \\ \hline
\multirow{3}{*}{\textbf{dorothea}} & \textbf{preprocessors} & -                  & -                                                                                    &                   & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & RandomForest                                                                         & DecisionTree      & -                 & RandomForest       \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & \textbf{95.36}                                                                       & {\ul 94.78}       & -                 & \textbf{95.36}     \\ \hline
\multirow{3}{*}{\textbf{gcredit}}  & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{accuracy}      & -                  & -                                                                                    & -                 & -                 & -                  \\ \hline
\multirow{3}{*}{\textbf{gisette}}  & \textbf{preprocessors} & -                  & -                                                                                    & -                 & -                 & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & LogisticRegression & -                                                                                    & -                 & -                 & LogisticRegression \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{97.29}     & -                                                                                    & -                 & -                 & {\ul 97.19}        \\ \hline
\multirow{3}{*}{\textbf{shuttle}}  & \textbf{preprocessors} & ZeroCount          & -                                                                                    & -                 & SelectPercentile  & -                  \\ \cline{2-7} 
                                   & \textbf{predictor}     & XGBoost            & ExtraTrees                                                                           & RandomForest      & RandomForest      & GradientBoosting   \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{99.99}     & \textbf{99.99}                                                                       & \textbf{99.99}    & \textbf{99.99}    & \textbf{99.99}     \\ \hline
\multirow{3}{*}{\textbf{wineqw}}   & \textbf{preprocessors} & PolynomialFeatures & \begin{tabular}[c]{@{}l@{}}VarianceThreshold $\rightarrow$\\ StackingEstimator\end{tabular} & StackingEstimator & StackingEstimator & PolynomialFeatures \\ \cline{2-7} 
                                   & \textbf{predictor}     & ExtraTrees         & RandomForest                                                                         & ExtraTrees        & GradientBoosting  & ExtraTrees         \\ \cline{2-7} 
                                   & \textbf{accuracy}      & \textbf{64.26}     & 58.13                                                                                & 62.70             & 58.00             & {\ul 58.07}        \\ \hline
\end{tabular}

\caption {Pipeline structure and accuracy in percentage generated by TPOT using different datasets and seed numbers}
\label{tab:tpot_exp}
\vspace{-0.5cm}
\end{table*}


\end{landscape}
